ChatGPT Hallucinates when Attributing Answers

Can ChatGPT provide evidence to support its answers? Does the evidence it suggests actually exist and does it really support its answer? We investigate these questions using a collection of domain-specific knowledge-based questions, specifically prompting ChatGPT to provide both an answer and supporting evidence in the form of references to external sources. We also investigate how different prompts impact answers and evidence. We find that ChatGPT provides correct or partially correct answers in about half of the cases (50.6% of the times), but its suggested references only exist 14% of the times. We further provide insights on the generated references that reveal common traits among the references that ChatGPT generates, and show how even if a reference provided by the model does exist, this reference often does not support the claims ChatGPT attributes to it. Our findings are important because (1) they are the first systematic analysis of the references created by ChatGPT in its answers; (2) they suggest that the model may leverage good quality information in producing correct answers, but is unable to attribute real evidence to support its answers. Prompts, raw result files and manual analysis are made publicly available.

==> Sections/4_experiment-settings.tex <==
\section{Experiment Settings}

As questions to submit to ChatGPT, we use the topics from the Ag-valuate collection~\cite{koopman2023agask}, a test collection for both passage and document retrieval in the Agriculture domain. The topics consist of natural language questions created by agricultural scientists and crop growers, and the collection contains a total of 160 topics\footnote{We only used the training portion of the topics for our experiments.}. Along with questions, the collection also provides a topic-creator authored answer, which forms the ground truth, and sparse relevance judgements over a dataset of 9M+ passages extracted from specialised agricultural websites and scientific publications. An example question and ground truth answer is shown in Figure~\ref{fig-sample}.
%Topics covered included recommendations and research relevant to the management of individual crops through varietals selection, sowing times, planting rates and row spacing, etc.; whole farming system performance, crop sequencing and fallow management practices; fertiliser management; and the identification and management of pest and diseases that affected the grains industry. 


\begin{figure}
	\ttfamily  \raggedright
	Consider my question: {[question\_text]} \\[4pt]
	Now, provide evidence for my question, for example research articles, articles from specialised magazines, Wikipedia pages. If referencing a research article or magazine, provide the name of authors, title of the artitle, publication venue (including volume, issue, page numbers), year. If referencing Wikipedia or a web page, provide the page name and the URL. 
	\caption{GPTChat prompt format.}
	\label{fig-prompt}
\end{figure}

Questions were issued to the online version of ChatGPT (GPT3.5 version), and answers collected. In issuing questions, we embedded them into the simple prompt of Figure~\ref{fig-prompt}, which instructs the model to answer the question and provide evidence for the answer.


ChatGPT's answers were examined by the first two authors of the paper along with a research assistant, all computer scientist. This group of assessors were responsible to identify whether the answer contained references, and if it did, then they went on to locate the evidence, if it existed. Subsequently, a fourth annotator, the third author of this paper, analysed once again the answers. This annotator is an agricultural scientist in a leading university in Ag-Tech, and is expert in the crops -- the topic area the questions in the Ag-valuate collection focus on.
This annotator validated the previous annotations, correcting for errors. In addition, she validated the answers of ChatGPT for correctness and provided further comments regarding the model's answers. Finally, she also examined the references that were included in ChatGPT's answers and that we successfully located. For each of these, she assessed whether the reference contained the claims ChatGPT made with its regards. 


==> Sections/5_results_copy_2.tex <==
\section{Results}
\begin{table*}[]
    \centering
    \begin{tabular}{c|c|c|c|c|c|c|c|c|c}

          \hline
          &NFCorpus &  TREC-COVID & NQ & HotpotQA & FiQA & ArguAna & DBPedia & SciDocs & SciFact\\
          \hline
          
         Per-Query Frechet (4) & 0.0 & -0.5 & -0.056 &-0.389  &-0.444 & -0.222 & -0.333 & -0.389& -0.333\\
         Binary entropy (5) &  0.778 & -0.778& 0.167 & 0.556& 0.056 & 0.278 & 0.444 & 0.389 &0.556\\
         \hline
         
         
    \end{tabular}
    \caption{Kendall Tau Correlation value }
    \label{tab:my_label}
\end{table*}


==> Sections/extra.tex <==

\begin{table*}[t]
    \centering
    \begin{tabular}{c|c|c|c|c|c|c|c|c|c|c|c}

          \hline
          &NFCorpus &  TREC-COVID & NQ & HotpotQA & FiQA & ArguAna & DBPedia & SciDocs & SciFact & Quora& \textbf{Avrg}\\
          \hline
         Query Similarity (2) & 0.5 & 0.667 & 0.5 &   0.333 & 0.444 & 0.056 & 0.167 & 0.333 & 0.222 & 0.222 & 0.344
         \\
         % 0.389& 0.722& 0.5& 0.333& 0.444& 0.167 &  0.222&0.333& 0.222 & 0.222 & 0.356
         % \\
         Per-Corpus Frechet (3) &
         -0.222 & -0.5 & -0.444 & -0.333 &  -0.556 &-0.222 & -0.167 & -0.444 &-0.389 & -0.556 & -0.383
         % -0.111 & -0.5 & -0.444 & -0.333 &  -0.556 & -0.278 & -0.222&-0.444 & -0.389 & -0.556 & -0.372
         \\          
         % Per-Query Frechet (4) & 0.0 & -0.5 & -0.056 &-0.389  &-0.444 & -0.222 & -0.333 & -0.389& -0.333 & -0.5 & -0.317\\
         Binary entropy (5) &  0.278  & -0.444 &  0.389  & 0.444 & 0.0 &  0.389 &  &  0.389 & 0.5 & 0.333 &  \\
         
         \hline
         
    \end{tabular}
    \caption{Kendall Tau Correlation value, calculated based on MAP }
    \label{tab:tau_MAP@1000}
\end{table*}
